Snitch: A tiny Pseudo Dual-Issue Processor for Area and Energy Efficient Execution of Floating-Point Intensive Workloads

Data-parallel applications, such as data analytics, machine learning, and scientific computing, are placing an ever-growing demand on floating-point operations per second on emerging systems. With increasing integration density, the quest for energy efficiency becomes the number one design concern. While dedicated accelerators provide high energy efficiency, they are over-specialized and hard to adjust to algorithmic changes. We propose an architectural concept that tackles the issues of achieving extreme energy efficiency while still maintaining high flexibility as a general-purpose compute engine. The key idea is to pair a tiny 10kGE control core, called Snitch, with a double-precision FPU to adjust the compute to control ratio. While traditionally minimizing non-FPU area and achieving high floating-point utilization has been a trade-off, with Snitch, we achieve them both, by enhancing the ISA with two minimally intrusive extensions: stream semantic registers (SSR) and a floating-point repetition instruction (FREP). SSRs allow the core to implicitly encode load/store instructions as register reads/writes, eliding many explicit memory instructions. The FREP extension decouples the floating-point and integer pipeline by sequencing instructions from a micro-loop buffer. These ISA extensions significantly reduce the pressure on the core and free it up for other tasks, making Snitch and FPU effectively dual-issue at a minimal incremental cost of 3.2%. The two low overhead ISA extensions make Snitch more flexible than a contemporary vector processor lane, achieving a $2\times$ energy-efficiency improvement. We have evaluated the proposed core and ISA extensions on an octa-core cluster in 22nm technology. We achieve more than $5\times$ multi-core speed-up and a $3.5\times$ gain in energy efficiency on several parallel microkernels.

==> tables/isa_overview.tex <==
\begin{table}[]
    \caption{Different \glspl{isa} and their implementation of repetition instructions.}
    \begin{tabularx}{\linewidth}{@{}lll@{}}
        \toprule
        \gls{isa}                           & Present & Description                                                              \\\midrule
        X86~\cite{intelisa2016}             & Yes     & REP*: Repeat a single instruction conditionally (based on status flags). \\
        Arm~\cite{arm2018}                  & No      & ---                                                                      \\
        RISC-V~\cite{waterman2014risc}      & No      & ---                                                                      \\
        Power~\cite{powerisa2010}           & No      & ---                                                                      \\
        MIPS~\cite{mips2016}                & No      & ---                                                                      \\
        Sparc~\cite{sparc2016}              & No      & ---                                                                      \\
        Arc~\cite{arc2010}                  & No      & ---                                                                      \\
        TMS320C28x~\cite{tms320c28x2004cpu} & Yes     & RPT: Repeat a single instruction $n$ times based on a register value.    \\
        \bottomrule
    \end{tabularx}
    \label{tab:isa_overview}
\end{table}
